Quasi-perfect Lee Codes of Radius 2 and Arbitrarily Large Dimension

A construction of 2-quasi-perfect Lee codes is given over the space $\mathbb Z_p^n$ for $p$ prime, $p\equiv \pm 5\pmod{12}$ and $n=2[\frac{p}{4}]$. It is known that there are infinitely many such primes. Golomb and Welch conjectured that perfect codes for the Lee-metric do not exist for dimension $n\geq 3$ and radius $r\geq 2$. This conjecture was proved to be true for large radii as well as for low dimensions. The codes found are very close to be perfect, which exhibits the hardness of the conjecture. A series of computations show that related graphs are Ramanujan, which could provide further connections between Coding and Graph Theories.

==> gaussian.tex <==
\section{Gaussian Integers}\label{appendix:gaussianos}%si usando comando \appendices

For more details on the ring of Gaussian integers the book by Hardy and Wright~\cite{Hardy} is a classical reference. In this Appendix some standard definitions and results
on Gaussian integers are summarized, for the completeness of the article.

The set of the \textsl{Gaussian integers}
$$\mathbb Z[i]=\{a+bi\mid a,b\in\mathbb Z\}$$

is the extension of the integers by a symbol $i$, satisfying $i^2+1=0$. Given an element $\gamma=a+bi\in\mathbb Z[i]$, its \textsl{conjugate} is defined as $\gamma^*=a-bi$.
Then, the \textsl{norm} is defined as $\mathcal N(\gamma)=\gamma\gamma^*=a^2+b^2$. Thus, this norm is a function from $\mathbb Z[i]$ into $\mathbb Z$. Furthermore, the norm makes $\mathbb{Z}[i]$ an Euclidean domain, since for any $\alpha,\beta\neq 0\in\mathbb Z[i]$, there exist $\kappa,\rho\in\mathbb Z[i]$ such that $\alpha=\kappa\beta+\rho$ with $\mathcal N(\rho)\leq \frac{1}{2}\mathcal N(\beta)<\mathcal N(\beta)$.
The norm is multiplicative, this is, $\mathcal N(\alpha\beta)=\mathcal N(\alpha)\mathcal N(\beta)$.
Also, as conjugation is an involution, the norm of a Gaussian integer is equal to the norm of its conjugate, that is, $\mathcal N(\gamma^*)=\gamma^*(\gamma^*)^*=\gamma^*\gamma=\mathcal N(\gamma)$.
For a Gaussian integer $\gamma=a+bi$, let us define its real part $\Re(\gamma)=a=\frac{\gamma+\gamma^*}{2}$ and its imaginary part $\Im(\gamma)=b=\frac{\gamma-\gamma^*}{2i}$.
Both $\Re$ and $\Im$ are also functions from $\mathbb Z[i]$ into $\mathbb Z$.

Since the Gaussian integers are an Euclidean domain, they also form a principal ideal domain and a unique factorization domain.
The four units of $\mathbb Z[i]$ are $\{1,i,-1,-i\}$ and the uniqueness of factorization is considered up to commutativity and multiplication by these units.
If two Gaussian integers have the same factorization, then they are said to be \textsl{associates}. Now, Gaussian primes fall into two categories:
\begin{itemize}
\item $\alpha=p$ for some $p\in\mathbb Z$ prime over the integers satisfying $p\equiv 3\pmod 4$. Its norm is $\mathcal N(\alpha)=p^2$.
\item $\alpha=a+bi$ with norm $\mathcal N(\alpha)=a^2+b^2=p$ for some integer prime $p$. This integer must satisfy $p=2$ or $p\equiv 1\pmod 4$.
\end{itemize}

Given a Gaussian integer $\alpha\in\mathbb Z[i]$, the quotient ring $\mathbb Z[i]/\alpha\mathbb Z[i]$ can be considered. This is, if for $\gamma_1,\gamma_2\in\mathbb Z[i]$, their difference is a multiple of $\alpha$, then $\gamma_1\equiv \gamma_2\pmod \alpha$ and $\gamma_1,\gamma_2$ are representatives of the same element in $\mathbb Z[i]/\alpha\mathbb Z[i]$.
The number of elements of the quotient ring $\mathbb Z[i]/\alpha\mathbb Z[i]$ is $\mathcal N(\alpha)$.
When $\alpha$ is a Gaussian prime, the quotient ring is also a field; otherwise, the divisors of $\alpha$ become representatives of zero divisor elements in the quotient.

The special case of $\mathbb Z[i]/p\mathbb Z[i]$ for some integer prime $p$ has interesting consequences. The cardinal is always $p^2$. Then, the ring is a field if and only if $p\equiv 3\pmod 4$.
The Gaussian norm becomes a function $\mathcal N:\mathbb Z[i]/p\mathbb Z[i]\longrightarrow  \mathbb Z/p\mathbb Z$;
and $\mathbb Z/p\mathbb Z$ is always a field. Finally, the norm of an element is 0 if and only if it is a zero divisor.


